Finite-Time Analysis for Double Q-learning

Although Q-learning is one of the most successful algorithms for finding the best action-value function (and thus the optimal policy) in reinforcement learning, its implementation often suffers from large overestimation of Q-function values incurred by random sampling. The double Q-learning algorithm proposed in~\citet{hasselt2010double} overcomes such an overestimation issue by randomly switching the update between two Q-estimators, and has thus gained significant popularity in practice. However, the theoretical understanding of double Q-learning is rather limited. So far only the asymptotic convergence has been established, which does not characterize how fast the algorithm converges. In this paper, we provide the first non-asymptotic (i.e., finite-time) analysis for double Q-learning. We show that both synchronous and asynchronous double Q-learning are guaranteed to converge to an $\epsilon$-accurate neighborhood of the global optimum by taking $\tilde{\Omega}\left(\left( \frac{1}{(1-\gamma)^6\epsilon^2}\right)^{\frac{1}{\omega}} +\left(\frac{1}{1-\gamma}\right)^{\frac{1}{1-\omega}}\right)$ iterations, where $\omega\in(0,1)$ is the decay parameter of the learning rate, and $\gamma$ is the discount factor. Our analysis develops novel techniques to derive finite-time bounds on the difference between two inter-connected stochastic processes, which is new to the literature of stochastic approximation.

==> Double Q-learning_NIPS20/SupplementaryBC.tex <==
\section{Proof of Theorem \ref{thm:asyncDQ} }\label{app:asyncThm}

The main idea of this proof is similar to that of Theorem \ref{thm:syncDQ} with further efforts to characterize the effects of asynchronous sampling. The proof also consists of three parts: (a) Part I which analyzes the stochastic error propagation between the two Q-estimators $\norm{Q^B_t  - Q^A_t }$; (b) Part II which analyzes the error dynamics between one Q-estimator and the optimum $\norm{Q^A_t -Q^* }$ conditioned on the error event in Part I; and (c) Part III which bounds the unconditional error $\norm{Q^A_t -Q^*}$.
% However, additional work has to be done to characterize the effects of asynchronous sampling. 

To proceed the proof,  we first introduce the following notion of valid iterations for any fixed state-action pair $(s,a)$.

\begin{definition}\label{def:TAsa}
We define $T(s,a)$ as the collection of iterations if a state-action pair $(s,a)$ is used to update the Q-function $Q^A$ or $Q^B$, and $T^A(s, a)$ as the collection of iterations specifically updating $Q^A(s,a)$. In addition, we denote $T(s, a, t_1, t_2)$ and $T^A(s, a, t_1, t_2)$ as the set of iterations updating $(s,a)$ and $Q^A(s,a)$ between time $t_1$ and $t_2$, respectively. That is, 
\begin{align*}
    T(s, a, t_1, t_2) &= \left\{ t: t\in [t_1, t_2] \text{ and } t\in T(s,a) \right\},\\
    T^A(s, a, t_1, t_2) &= \left\{ t: t\in [t_1, t_2] \text{ and } t\in T^A(s,a) \right\}.
\end{align*}
Correspondingly, the number of iterations updating $(s,a)$ between time $t_1$ and $t_2$ equals the cardinality of $T(s, a, t_1, t_2)$ which is denoted as $|T(s, a, t_1, t_2)|$. Similarly, the number of iterations updating $Q^A(s,a)$ between time $t_1$ and $t_2$ is denoted as $|T^A(s, a, t_1, t_2)|$.
\end{definition}

Given Assumption \ref{asp:covering}, we can obtain some properties of the quantities defined above.
\begin{lemma}\label{prop:sa2L}
It always holds that $|T(s,a,t_1,t_2)|\leq t_2-t_1+1$ and $|T^A(s,a,t_1,t_2)|\leq t_2-t_1+1$. In addition, suppose that Assumption \ref{asp:covering} holds. Then we have $T(s,a,t,t+2kL-1)\geq k$ for any $t\geq 0$.
\end{lemma}
\begin{proof}
Since in a consecutive $2L$ running iterations of Algorithm \ref{alg:doubleQ}, either $Q^A$ or $Q^B$ is updated at least $L$ times. Then following from Assumption \ref{asp:covering}, $(s,a)$ is visited at least once for each $2L$ running iterations of Algorithm \ref{alg:doubleQ}, which immediately implies this proposition.
\end{proof}

%In the remaining, we will use the quantities in Definition \ref{def:TAsa} and Assumption \ref{asp:covering} to show the result for asynchronous double Q-learning.
Now we proceed our proof by three parts.

\subsection{Part I: Bounding $\norm{Q^B_t-Q^A_t}$} \label{subsec:PartIThm2}

We upper bound $\norm{Q^B_t - Q^A_t}$ block-wisely using a decreasing sequence $\{G_q\}_{q\geq0}$ as defined in~\Cref{lem:GqAsy} below.
\begin{proposition}\label{lem:GqAsy}
Fix $\epsilon>0, \kappa\in(\ln 2,1)$ and $\Delta\in(0, e^{\kappa}-2)$. Consider asynchronous double Q-learning using a polynomial learning rate $\alpha_t = \frac{1}{t^\omega}$ with $\omega\in(0,1)$. Suppose that Assumption \ref{asp:covering} holds. Let $G_q = (1-\xi)^q G_0$ with $G_0 = V_{\max}$ and $\xi=\frac{1-\gamma}{4}$. Let $\hat{\tau}_{q+1} = \hat{\tau}_q + \frac{2cL}{\kappa}\hat{\tau}_q^\omega$ for $q \geq 1$ with $c\geq \frac{L\kappa(\ln(2+\Delta) + 1/\tau_1^\omega)}{2(\kappa-\ln(2+\Delta) - 1/\tau_1^\omega)}$ and $\hat{\tau}_1$ as the finishing time of the first block satisfying 
\begin{equation*}
    \hat{\tau}_1\geq  \max\left\{\left(\frac{1}{\kappa-\ln(2+\Delta)}\right)^{\frac{1}{\omega}}, \left( \frac{128cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\xi^2\sigma^2\epsilon^2 }\ln\left(\frac{64cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\xi^2\sigma^2\epsilon^2 }\right) \right)^{\frac{1}{\omega}} \right\}.
\end{equation*}
Then for any $n$ such that $G_n\geq\sigma\epsilon$, we have
\begin{align*}
    &\mP\left[ \forall q\in [0,n], \forall t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2}), \norm{Q^B_t - Q^A_t}\leq G_{q+1} \right]\\
    &\quad\geq 1- \frac{4cL(n+1)}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64cL(cL+\kappa)V_{\max}^2} \right).
\end{align*}
\end{proposition}
The proof of~\Cref{lem:GqAsy} consists of the following steps. Since the main idea of the proofs is similar to that of~\Cref{lem:Gq}, we will focus on pointing out the difference. We continue to use the notation $u^{BA}_t(s,a):=Q^B_t(s,a)-Q^A_t(s,a)$.

\textbf{Step 1: Characterizing the dynamics of $u^{BA}_t$}

First, we observe that when $(s,a)$ is visited at time $t$, i.e., $t\in T(s,a)$, Lemmas \ref{lem:uBAdyn} and \ref{lem:uBAsanwich} still apply. Otherwise, $u^{BA}$ is not updated. Thus, we have
\begin{equation*}
    u_{t+1}^{BA}(s,a) = \left\{\begin{aligned} 
    &u_t^{BA}(s,a),\quad t\notin T(s,a);\\
    &(1-\alpha_t)u_t^{BA}(s,a) + \alpha_t F_t(s,a),\quad t\in T(s,a),
    \end{aligned}\right.
\end{equation*}
where $F_t$ satisfies
\begin{equation*}
    \norm{\mE[F_t|\mcF_t]} \leq \frac{1+\gamma}{2} \norm{u_t^{BA}}.
\end{equation*}
For $t\in T(s,a)$, we rewrite the dynamics of $u_t^{BA}(s,a)$ as
\begin{equation*}
    u_{t+1}^{BA}(s,a) = (1-\alpha_t)u_t^{BA}(s,a) + \alpha_t F_t = (1-\alpha_t)u_t^{BA}(s,a) + \alpha_t (h_t(s,a) + z_t(s,a)),
\end{equation*}
where $h_t(s,a) = \mE[F_t(s,a)|\mcF_t]$ and $z_t(s,a) = F_t(s,a) - \mE[F_t(s,a)|\mcF_t]$. 

In the following steps, we use induction to proceed the proof of~\Cref{lem:GqAsy}. Given $G_q$ defined in~\Cref{lem:GqAsy}, since $\norm{u_t^{BA} }\leq G_0$ holds for all $t$, and thus it holds for $t\in [0,\hat{\tau}_1]$. Now suppose $\hat{\tau}_q$ satisfies that $\norm{u_t^{BA} }\leq G_q$ for any $t\geq \hat{\tau}_q$. Then we will show there exists $\hat{\tau}_{q+1} = \hat{\tau}_q + \frac{2cL}{\kappa}\hat{\tau}_q^\omega$ such that $\norm{u_t^{BA} }\leq G_{q+1}$ for any $t\geq \hat{\tau}_{q+1}$.

\textbf{Step 2: Constructing sandwich bounds}

We first observe that the following sandwich bound still holds for all $t\geq \hat{\tau}_q$.
\begin{equation*}
    -X_{t;\hat{\tau}_q}(s,a) + Z_{t;\hat{\tau}_q}(s,a) \leq u_t^{BA}(s,a) \leq X_{t;\hat{\tau}_q}(s,a) + Z_{t;\hat{\tau}_q}(s,a),
\end{equation*}
where $Z_{t;\hat{\tau}_q}(s,a)$ is defined as
\begin{equation*}
    Z_{t+1;\hat{\tau}_q}(s,a) = \left\{\begin{aligned}
    & Z_{t;\hat{\tau}_q}(s,a), \quad t\notin T(s,a)\\
    & (1-\alpha_t)Z_{t;\hat{\tau}_q}(s,a) + \alpha_t z_t(s,a), \quad t\in T(s,a),
    \end{aligned}
    \right.
\end{equation*}
with the initial condition $Z_{\hat{\tau}_q;\hat{\tau}_q}(s,a) = 0$, and $X_{t;\hat{\tau}_q}(s,a)$ is defined as
\begin{equation*}
    X_{t+1;\hat{\tau}_q}(s,a) = \left\{\begin{aligned}
    & X_{t;\hat{\tau}_q}(s,a), \quad t\notin T(s,a)\\
    & (1-\alpha_t)X_{t;\hat{\tau}_q}(s,a) + \alpha_t \gamma'G_q, \quad t\in T(s,a),
    \end{aligned}
    \right.
\end{equation*}
with $X_{\hat{\tau}_q;\hat{\tau}_q}(s,a) = G_q,\gamma'=\frac{1+\gamma}{2}$.

This claim can be shown by induction. This bound clearly holds for the initial case with $t=\hat{\tau}_q$. Assume that it still holds for iteration $t$. If $t\in T(s,a)$, the proof is the same as that of~\Cref{lem:uBAsanwich}. If $t\notin T(s,a)$, since all three sequences do not change from time $t$ to time $t+1$, the sandwich bound still holds. Thus we conclude this claim.

\textbf{Step 3: Bounding $X_{t;\hat{\tau}_q}(s,a)$}

Next, we bound the deterministic sequence $X_{t;\hat{\tau}_q}(s,a)$. Observe that $X_{t;\hat{\tau}_q}(s,a)\leq G_q$ for any $t\geq\hat{\tau}_q$. We will next show that $X_{t;\hat{\tau}_q}(s,a) \leq \left(\gamma' + \frac{2}{2+\Delta}\xi\right)G_q$ for any $t\in [\hat{\tau}_{q+1},\hat{\tau}_{q+2})$ where $\hat{\tau}_{q+1} = \hat{\tau}_q + \frac{2cL}{\kappa}\hat{\tau}_q^\omega$. 

Similarly to the proof of~\Cref{lem:Xt}, we still rewrite $X_{\hat{\tau}_q;\hat{\tau}_q}(s,a)$ as $X_{\hat{\tau}_q;\hat{\tau}_q}(s,a) = G_q = \gamma' G_q + (1-\gamma')G_q := \gamma' G_q + \rho_{\hat{\tau}_q} $. However, in this case the dynamics of $X_{t;\hat{\tau}_q}(s,a)$ is different, which is represented as
\begin{equation*}
    X_{t+1;\hat{\tau}_q}(s,a) =\left\{\begin{aligned} 
    & X_{t;\hat{\tau}_q}(s,a), \quad t\notin T(s,a)\\
    &(1-\alpha_t)X_{t;\hat{\tau}_q}(s,a) + \alpha_t \gamma'G_q = \gamma'G_q + (1-\alpha_t)\rho_t, \quad t\in T(s,a).
    \end{aligned}
    \right.
\end{equation*}
where $\rho_{t+1} = (1-\alpha_t)\rho_t$ when $t\in T(s,a)$. By the definition of $\rho_t$, we obtain
\begin{align*}
    \rho_t &= \rho_{\hat{\tau}_q}\underset{i\in T(s, a, \hat{\tau}_q, t-1)}{\Pi}(1-\alpha_i) 
    = (1-\gamma')G_q\underset{i\in T(s, a, \hat{\tau}_q, t-1)}{\Pi}(1-\alpha_i)\\
    &\leq (1-\gamma')G_q\underset{i\in T(s, a, \hat{\tau}_q, \hat{\tau}_{q+1}-1)}{\Pi}\left(1-\frac{1}{i^\omega}\right) 
    \leq (1-\gamma')G_q\prod_{i=\hat{\tau}_{q+1}-|T(s, a, \hat{\tau}_q, \hat{\tau}_{q+1}-1)|}^{\hat{\tau}_{q+1}-1}\left(1-\frac{1}{i^\omega}\right)\\
    &\overset{\text{(i)}}{\leq} (1-\gamma')G_q\prod_{i=\hat{\tau}_{q+1}-\frac{c}{\kappa}\hat{\tau}_q^\omega}^{\hat{\tau}_{q+1}-1}\left(1-\frac{1}{i^\omega}\right)
    \overset{\text{(ii)}}{\leq} (1-\gamma')G_q\exp\left( -\frac{\frac{c}{\kappa}\hat{\tau}_q^\omega-1}{(\hat{\tau}_{q+1}-1)^\omega} \right)\\
    &\leq (1-\gamma')G_q\exp\left( -\frac{\frac{c}{\kappa}\hat{\tau}_q^\omega-1 }{\hat{\tau}_{q+1}^\omega} \right)
    = (1-\gamma')G_q\exp\left( -\frac{c}{\kappa}\left(\frac{\hat{\tau}_q}{\hat{\tau}_{q+1}}\right)^\omega + \frac{1}{\hat{\tau}_{q+1}^\omega} \right)\\
    &\overset{\text{(iii)}}{\leq} (1-\gamma')G_q\exp\left( -\frac{c}{\kappa}\frac{1}{1+\frac{2cL}{\kappa}} + \frac{1}{\hat{\tau}_{1}^\omega} \right),
\end{align*}
where (i) follows from~\Cref{prop:sa2L}, (ii) follows~\Cref{lem:prodHelp}, and (iii) follows because $\hat{\tau}_q\geq\hat{\tau}_1$ and
\begin{equation*}
    \left(\frac{\hat{\tau}_q}{\hat{\tau}_{q+1}}\right)^\omega \geq \frac{\hat{\tau}_q}{\hat{\tau}_{q+1}} = \frac{\hat{\tau}_q}{\hat{\tau}_{q} + \frac{2cL}{\kappa}\hat{\tau}_q^\omega}\geq \frac{1}{1+\frac{2cL}{\kappa}}.
\end{equation*}

Since $\kappa\in(\ln 2,1)$ and $\Delta\in(0, e^{\kappa}-2)$, we have $\ln (2+\Delta)\in (0, \kappa)$. Further, observing $\hat{\tau_1}^\omega > \frac{1}{\kappa-\ln(2+\Delta)}$, we obtain $\ln(2+\Delta) + \frac{1}{\hat{\tau_1}^\omega} \in (0,\kappa)$. Last, since $c\geq\frac{L\kappa(\ln(2+\Delta) + 1/\hat{\tau_1}^\omega)}{2(\kappa-\ln(2+\Delta) - 1/\hat{\tau_1}^\omega)}$, we have $-\frac{c}{1+\frac{2c}{\kappa}} + \frac{1}{\hat{\tau_1}^\omega}\leq -\ln(2+\Delta)$.

Finally, combining the above observations with the fact $1-\gamma'=2\xi$, we conclude that for any $t\geq \hat{\tau}_{q+1} = \hat{\tau}_q + \frac{2cL}{\kappa}\hat{\tau}_q^\omega$,
\begin{equation*}
    X_{t;\hat{\tau}_q}(s,a) \leq \left(\gamma' + \frac{2}{2+\Delta}\xi\right)G_q.
\end{equation*}

\textbf{Step 4: Bounding $Z_{t;\hat{\tau}_q}(s,a)$}

It remains to bound the stochastic sequence $Z_{t;\hat{\tau}_q}(s,a)$ by $\frac{\Delta}{2+\Delta}\xi G_q$ at epoch $q+1$. We define an auxiliary sequence $\{Z_{t;\hat{\tau}_q}^l (s,a)\}$ (which is different from that in \eqref{eq:Zl}) as:
\begin{equation*}
    Z^l_{t;\hat{\tau}_q}(s,a) = \sum_{i\in T(s, a, \hat{\tau}_q, t-1)}\alpha_i\underset{j\in T(s, a, i+1, t-1)}{\Pi}(1-\alpha_j) z_i(s,a).
\end{equation*}
Following the same arguments as the proof of Lemma \ref{lem:ZlDiff}, we conclude that $\{Z_{t;\hat{\tau}_q}^l (s,a)\}$ is a martingale sequence and satisfies
\begin{equation*}
    \lvert Z^l_{t;\hat{\tau}_q}(s,a) - Z^{l-1}_{t;\hat{\tau}_q}(s,a) \rvert = \alpha_{\hat{\tau}_q+l} |z_{\hat{\tau}_q + l}(s,a)|\leq \frac{2V_{\max}}{\hat{\tau}_q^\omega}.
\end{equation*}

In addition, note that 
\begin{align*}
    Z_{t;\hat{\tau}_q}(s,a) &= Z_{t;\hat{\tau}_q}(s,a) - Z_{\hat{\tau}_q;\hat{\tau}_q}(s,a)\\
    &= \sum_{l:\hat{\tau}_q+l-1\in T(s, a, \hat{\tau}_q, t-1)} (Z^l_{t;\hat{\tau}_q}(s,a) - Z^{l-1}_{t;\hat{\tau}_q}(s,a)) + Z^{\min(T(s, a, \hat{\tau}_q, t-1))}_{t;\hat{\tau}_q}(s,a).
\end{align*}
Then we apply Azuma' inequality in Lemma \ref{lem:azuma} and obtain
\begin{align*}
    &\mP\left[ \lvert Z_{t;\hat{\tau}_q}(s,a)  \rvert > \hat{\epsilon}| t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2})  \right]\\
    &\quad\leq 2\exp\left( \frac{-\hat{\epsilon}^2}{2\underset{l:\hat{\tau}_q+l-1\in T(s, a, \hat{\tau}_q, t-1)}{\sum} (Z^l_{t;\hat{\tau}_q}(s,a) \!-\! Z^{l-1}_{t;\hat{\tau}_q}(s,a))^2 \!+\! 2\left(Z^{\min(T(s, a, \hat{\tau}_q, t-1))}_{t;\hat{\tau}_q}(s,a)\right)^2} \right)\\
    &\quad\leq 2\exp\left( -\frac{\hat{\epsilon}^2\hat{\tau}_q^{2\omega}}{8(|T(s, a, \hat{\tau}_q, t-1)|+1) V_{\max}^2} \right) 
    \overset{\text{(i)}}{\leq} 2\exp\left( -\frac{\hat{\epsilon}^2\hat{\tau}_q^{2\omega}}{8(t-\hat{\tau}_q)  V_{\max}^2} \right)\\
    &\quad\leq 2\exp\left( -\frac{\hat{\epsilon}^2\hat{\tau}_q^{2\omega}}{8(\hat{\tau}_{q+2}-\hat{\tau}_q)  V_{\max}^2} \right) 
    = 2\exp\left( -\frac{\hat{\epsilon}^2\hat{\tau}_q^{2\omega}}{8 \left(\frac{2cL}{\kappa}\hat{\tau}_{q+1}^\omega+\frac{2cL}{\kappa}\hat{\tau}_q^\omega\right) V_{\max}^2} \right)\\
    &\quad = 2\exp\left( -\frac{\hat{\epsilon}^2\hat{\tau}_q^{2\omega}}{8 \left(\frac{2cL}{\kappa}(\hat{\tau}_{q}+\frac{2cL}{\kappa}\hat{\tau}_q^\omega)^\omega+\frac{2cL}{\kappa}\hat{\tau}_q^\omega\right) V_{\max}^2} \right)\\
    &\quad\leq 2\exp\left( -\frac{\kappa^2\hat{\epsilon}^2\hat{\tau}_q^{\omega}}{32cL(cL+\kappa) V_{\max}^2} \right)
    % &\quad \leq 2\exp\left( -\frac{\kappa^2\hat{\epsilon}^2\hat{\tau}_q^{2\omega-p}}{32L(L+\kappa) V_{\max}^2} \right)
    % = 2\exp\left( -\frac{\kappa^2\hat{\epsilon}^2\hat{\tau}_q^{\frac{3\omega-1}{2}}}{32L(L+\kappa) V_{\max}^2} \right),
\end{align*}
where (i) follows from~\Cref{prop:sa2L}.

\textbf{Step 5: Taking union over all blocks}

Finally, using the union bound of~\Cref{lem:unionBound} yields
\begin{align*}
    &\mP\left[ \forall q\in [0,n], \forall t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2}), \norm{Q^B_t  - Q^A_t }\leq G_{q+1} \right]\\
    &\quad\geq \mP\left[ \forall(s,a), \forall q\in [0,n], \forall t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2}), \lvert Z_{t;\hat{\tau}_q}(s,a)  \rvert \leq \frac{\Delta}{2+\Delta}\xi G_q \right]\\
    &\quad\geq 1 - \sum_{q=0}^n |\mcs||\mca|(\hat{\tau}_{q+2} - \hat{\tau}_{q+1}) \cdot \mP\left[ \lvert Z_{t;\hat{\tau}_q}(s,a)  \rvert > \frac{\Delta}{2+\Delta}\xi G_q \Big\rvert t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2})  \right]\\
    &\quad\geq 1 - \sum_{q=0}^n |\mcs||\mca| \frac{2cL}{\kappa}\hat{\tau}_{q+1}^\omega \cdot 2\exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 G_q^2\hat{\tau}_q^{\omega}}{32cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\geq 1 - \sum_{q=0}^n |\mcs||\mca| \frac{2cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\hat{\tau}_{q}^\omega \cdot 2\exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 G_q^2\hat{\tau}_q^{\omega}}{32cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\overset{\text{(i)}}{\geq} 1 - \sum_{q=0}^n |\mcs||\mca| \frac{2cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\hat{\tau}_{q}^\omega \cdot 2\exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_q^{\omega}}{32cL(cL+\kappa)V_{\max}^2} \right)\\
    % &\quad= 1 - \sum_{q=0}^n |\mcs||\mca| \frac{2cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\left(\hat{\tau}_{q}^{\frac{3\omega-1}{2}}\right)^{\frac{2p}{3\omega-1}} \cdot 2\exp\left( -\frac{\kappa^2\left( 1-\frac{2}{e} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_q^{\frac{3\omega-1}{2}}}{32cL(L+\kappa)V_{\max}^2} \right)\\
    &\quad\overset{\text{(ii)}}{\geq} 1 - \frac{4cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\sum_{q=0}^n |\mcs||\mca| \cdot \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 
    \sigma^2\epsilon^2\hat{\tau}_q^{\omega}}{64cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\overset{\text{(iii)}}{\geq} 1- \frac{4cL(n+1)}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64cL(cL+\kappa)V_{\max}^2} \right),
\end{align*}
where (i) follows from $G_q \geq G_n \geq \sigma\epsilon $, (ii) follows from~\Cref{lem:tauHelp} by substituting $a=\frac{64cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\xi^2\sigma^2\epsilon^2 }, b=1$ and observing that
\begin{align*}
    \hat{\tau}_q^{\omega}&\geq\hat{\tau}_1^{\omega}\geq \frac{128cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\xi^2\sigma^2\epsilon^2 }\ln\left(\frac{64cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\xi^2\sigma^2\epsilon^2 }\right)=2ab\ln ab,
\end{align*}
and (iii) follows from $\hat{\tau}_q \geq \hat{\tau}_1$.

\subsection{Part II: Conditionally bounding $\norm{Q^A_t-Q^*}$} \label{subsec:PartIIThm2}
We upper bound $\norm{Q^A_t-Q^*}$ block-wisely by a decreasing sequence $\{D_k\}_{k\geq0}$ conditioned on the following two events: fix a positive integer $m$, 
\begin{align}
    G & = \left\{ \forall(s,a), \forall k\in [0,m], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^B_t  - Q^A_t }\leq \sigma D_{k+1} \right\}, \label{eq:eventE} \\
    H & = \{ \forall k\in [1,m+1], I^A_k\geq cL\tau_{k}^\omega \}, \label{eq:eventF}
\end{align}
where $I^A_k$ denotes the number of iterations updating $Q^A$ at epoch $k$, $\tau_k$ is the starting iteration index of the $k+1$th block, and $\omega$ is the parameter of the polynomial learning rate. Roughly, Event $G$ requires that the difference between the two Q-function estimators are bounded appropriately, and Event $H$ requires that $Q^A$ is sufficiently updated in each epoch. Again, we will design $\{D_k\}_{k\geq 0}$ in a way such that the occurrence of Event $G$ can be implied from the event that $\norm{u^{BA}_t}$ is bounded by $\{G_q\}_{q\geq 0}$ (see~\Cref{lem:coupleAsy} below). A lower bound of the probability for Event $H$ to hold is characterized in~\Cref{lem:halfQA} in Part III.
\begin{proposition}\label{lem:conditionalBoundAsy}
Fix $\epsilon>0, \kappa\in(\ln 2,1)$ and $\Delta\in(0, e^{\kappa}-2)$. Consider asynchronous double Q-learning using a polynomial learning rate $\alpha_t = \frac{1}{t^\omega}$ with $\omega\in(0,1)$. Let $\{G_q\}, \{\hat{\tau}_q\}$ be as defined in~\Cref{lem:GqAsy}. Define $D_k = (1-\beta)^k\frac{V_{\max}}{\sigma}$ with $\beta = \frac{1-\gamma(1+\sigma)}{2}$ and $\sigma = \frac{1-\gamma}{2\gamma}$. Let $\tau_k=\hat{\tau}_k$ for $k\geq0$.  Suppose that $c\geq \frac{L(\ln(2+\Delta) + 1/\tau_1^\omega)}{2(\kappa-\ln(2+\Delta) - 1/\tau_1^\omega)}$ and $\tau_1 = \hat{\tau}_1$ as the finishing time of the first epoch satisfies 
\begin{equation*}
    \tau_1\geq  \max\left\{\left(\frac{1}{\kappa-\ln(2+\Delta)}\right)^{\frac{1}{\omega}}, \left( \frac{32cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\beta^2\epsilon^2 }\ln \left(\frac{16cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\beta^2\epsilon^2 }\right) \right)^{\frac{1}{\omega}} \right\}.
\end{equation*}
Then for any $m$ such that $D_m\geq\epsilon$, we have
\begin{align*}
    &\mP\left[ \forall k\in [0,m], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^A_t  - Q^* }\leq D_{k+1} |G,H \right]\\
    &\quad\geq 1 - \frac{4cL(m+1)}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( 1-\frac{2}{e} \right)^2\beta^2 \epsilon^2\tau_1^{\omega}}{16cL(cL+\kappa)V_{\max}^2} \right).
\end{align*}
\end{proposition}
Recall that in the proof of~\Cref{lem:conditionalBound}, $Q^A$ is not updated at each iteration and thus we introduced notations $T^A$ and $T^A(t_1,t_2)$ in Definition \ref{def:TA} to capture the convergence of the error $\norm{Q^A -Q^* }$. In this proof, the only difference is that when choosing to update $Q^A$, only one $(s,a)$-pair is visited. Therefore, the proof of~\Cref{lem:conditionalBoundAsy} is similar to that of~\Cref{lem:conditionalBound}, where most of the arguments simply substitute $T^A, T^A(t_1,t_2)$ in the proof of~\Cref{lem:conditionalBound} by $T^A(s,a), T^A(s,a,t_1,t_2)$ in Definition \ref{def:TAsa}, respectively. Certain bounds are affected by such substitutions. In the following, we proceed the proof of~\Cref{lem:conditionalBoundAsy} in five steps, and focus on pointing out the difference from the proof of~\Cref{lem:conditionalBound}. More details can be referred to~\Cref{subsec:PartII}.


\textbf{Step 1: Coupling $\{D_k\}_{k\geq0}$ and $\{G_q\}_{q\geq0}$}

We establish the relationship between $\{D_k\}_{k\geq0}$ and $\{G_q\}_{q\geq0}$ in the same way as Lemma \ref{lem:couple}. For the convenience of reference, we restate \Cref{lem:couple} in the following.
\begin{lemma}\label{lem:coupleAsy}
Let $\{G_q\}$ be defined in~\Cref{lem:GqAsy}, and let $D_k = (1-\beta)^k\frac{V_{\max}}{\sigma}$ with $\beta = \frac{1-\gamma(1+\sigma)}{2}$ and $\sigma = \frac{1-\gamma}{2\gamma}$. Then we have
\begin{align*}
    &\mP\left[ \forall(s,a), \forall q\in [0,m], \forall t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2}), \norm{Q^B_t  - Q^A_t }\leq G_{q+1} \right]\\
    &\quad\leq \mP\left[ \forall(s,a), \forall k\in [0,m], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^B_t  - Q^A_t }\leq \sigma D_{k+1} \right],
\end{align*}
given that $\tau_k = \hat{\tau}_{k }$.
\end{lemma}


\textbf{Step 2: Constructing sandwich bounds}

Let $r_t(s,a)=Q^A(s,a)-Q^*(s,a)$ and $\tau_k$ be such that $\norm{r_t}\leq D_k$ for all $t\geq\tau_k$. The requirement of Event $G$ yields
\begin{equation*}
    -Y_{t;\tau_k}(s,a) + W_{t;\tau_k}(s,a) \leq r_t(s,a) \leq Y_{t;\tau_k}(s,a) + W_{t;\tau_k}(s,a),
\end{equation*}
where $W_{t;\tau_k}(s,a)$ is defined as
\begin{equation*}
    W_{t+1;\tau_k}(s,a) = \left\{\begin{aligned}
    &W_{t;\tau_k}(s,a), \quad t\notin T^A(s,a);\\
    &(1-\alpha_t)W_{t;\tau_k}(s,a) + \alpha_t w_t(s,a), \quad t\in T^A(s,a),
    \end{aligned}\right.
\end{equation*}
with $w_{t}(s,a) = \mcT_{t} Q_{t}^A(s,a) - \mcT Q_{t}^A(s,a)$ and $W_{\tau_k;\tau_k}(s,a) = 0$, and $Y_{t;\tau_k}(s,a)$ is given by
\begin{equation*}
    Y_{t+1;\tau_k}(s,a) = \left\{\begin{aligned}
    &Y_{t;\tau_k}(s,a), \quad t\notin T^A(s,a);\\
    &(1-\alpha_t)Y_{t;\tau_k}(s,a) + \alpha_t \gamma''D_k, \quad t\in T^A(s,a),
    \end{aligned}\right.
\end{equation*}
with $Y_{\tau_k;\tau_k}(s,a) = D_k$ and $\gamma''=\gamma(1+\sigma)$.

\textbf{Step 3: Bounding $Y_{t;\tau_k}(s,a)$}

Next, we first bound $Y_{t;\tau_k}(s,a)$. Observe that $Y_{t;\tau_k}(s,a) \leq D_k$ for any $t \geq \tau_k$. We will bound $Y_{t;\tau_k}(s,a)$ by $\left(\gamma'' + \frac{2}{2+\Delta}\beta\right)D_k$ for block $k+1$.

We use a similar representation of $Y_{t;\tau_k}(s,a)$ as in the proof of Lemma \ref{lem:Yt}, which is given by
\begin{equation*}
    Y_{t+1;\tau_k}(s,a) = \left\{\begin{aligned}
    & Y_{t;\tau_k}(s,a), \quad t\notin T^A(s,a)\\
    &(1-\alpha_t)Y_{t;\tau_k}(s,a) + \alpha_t \gamma''G_q = \gamma''G_q + (1-\alpha_t)\rho_t, \quad t\in T^A(s,a)
    \end{aligned}\right.
\end{equation*}
where $\rho_{t+1} = (1-\alpha_t)\rho_t$ for $t\in T^A(s,a)$. By the definition of $\rho_t$, we obtain
\begin{align*}
    \rho_t &= \rho_{\tau_k}\prod_{i\in T^A(s, a, \tau_k, t-1)}(1-\alpha_i) = (1-\gamma'')D_k\prod_{i\in T^A(s, a, \tau_k, t-1)}(1-\alpha_i)\\
    &= (1-\gamma'')D_k\prod_{i\in T^A(s, a, \tau_k, t-1)}\left(1-\frac{1}{i^\omega}\right) 
    \overset{\text{(i)}}{\leq} (1-\gamma'')D_k\prod_{i\in T^A(s, a, \tau_k, \tau_{k+1}-1)}\left(1-\frac{1}{i^\omega}\right)\\
    &\overset{\text{(ii)}}{\leq} (1-\gamma'')D_k\prod_{i=\tau_{k+1}-c\tau_k^\omega}^{\tau_{k+1}-1}\left(1-\frac{1}{i^\omega}\right)
    \overset{\text{(iii)}}{\leq} (1-\gamma'')D_k\exp\left( -\frac{c\tau_k^\omega-1}{(\tau_{k+1}-1)^\omega} \right) \nonumber\\
    &\leq (1-\gamma'')D_k\exp\left( -\frac{c\tau_k^\omega-1}{\tau_{k+1}^\omega} \right) 
    = (1-\gamma'')D_k\exp\left( -c\left(\frac{\tau_k}{\tau_{k+1}}\right)^\omega + \frac{1}{\tau_{k+1}^\omega} \right) \nonumber\\
    &\overset{\text{(iv)}}{\leq} (1-\gamma'')D_k\exp\left( -\frac{c}{1+\frac{2Lc}{\kappa}} + \frac{1}{\tau_{1}^\omega} \right), \nonumber
\end{align*}
where (i) follows because $\alpha_i<1$ and $t\geq \tau_{k+1}$, (ii) follows from Proposition \ref{prop:sa2L} and the requirement of event $H$, (iii) follows from Lemma \ref{lem:tauHelp}, and (iv) holds because $\tau+k\geq\tau_1$ and 
\begin{equation*}
    \left(\frac{\tau_k}{\tau_{k+1}}\right)^\omega \geq \frac{\tau_k}{\tau_{k+1}} = \frac{\tau_k}{\tau_{k} + \frac{2cL}{\kappa}\tau_k^\omega}\geq \frac{1}{1+\frac{2cL}{\kappa}}.
\end{equation*}
Since $\kappa\in(\ln 2,1)$ and $\Delta\in(0, e^{\kappa}-2)$, we have $\ln (2+\Delta)\in (0, \kappa)$. Further, observing $\hat{\tau_1}^\omega > \frac{1}{\kappa-\ln(2+\Delta)}$, we obtain $\ln(2+\Delta) + \frac{1}{\hat{\tau_1}^\omega} \in (0,\kappa)$. Last, since $c\geq\frac{L(\ln(2+\Delta) + 1/\hat{\tau_1}^\omega)}{2(\kappa-\ln(2+\Delta) - 1/\hat{\tau_1}^\omega)}$, we have $-\frac{c}{1+\frac{2c}{\kappa}} + \frac{1}{\hat{\tau_1}^\omega}\leq -\ln(2+\Delta)$.

Then, we have $\rho_t\leq \frac{1-\gamma''}{2+\Delta}D_k$. Thus we conclude that for any $t\in [\tau_{k+1}, \tau_{k+2}]$,
\begin{equation*}
    Y_{t;\tau_k}(s,a) \leq \left(\gamma'' + \frac{2}{2+\Delta}\beta\right)D_k.
\end{equation*}

\textbf{Step 4: Bounding $W_{t;\tau_k}(s,a)$}

It remains to bound $|W_{t;\tau_k}(s,a)|\leq \left(1-\frac{2}{2+\Delta}\right)\beta D_k$ for $t\in [\tau_{k+1},\tau_{k+2})$.

Similarly to \Cref{subsec:proofProp2}, we define a new sequence $\{W_{t;\tau_k}^l(s,a)\}$ as
\begin{equation*}
    W^l_{t;\tau_k}(s,a) = \sum_{i\in T^A(s, a, \tau_k, \tau_k+l)} \alpha_i\underset{j\in T^A(s, a, i+1, t-1)}{\Pi} (1-\alpha_j)w_i(s,a).
\end{equation*}
The same arguments as the proof of Lemma \ref{lem:WlDiff} yields
\begin{equation*}
    \lvert W^l_{t;\tau_k}(s,a) - W^{l-1}_{t;\tau_k}(s,a) \rvert \leq  \frac{V_{\max}}{\tau_k^\omega}.
\end{equation*}

If we fix $\tilde{\epsilon}>0$, then for any $t\in[\tau_{k+1},\tau_{k+2})$ we have
\begin{align*}
    &\mP\left[ |W_{t;\tau_k}(s,a)|>\tilde{\epsilon} | t\in[\tau_{k+1},\tau_{k+2}),G,H \right]\\
    &\leq 2\exp\left( \frac{-\tilde{\epsilon}^2}{2\underset{l:\tau_k+l-1\in T^A(s,a,\tau_k, t\!-\!1)}{\sum}\!\left( W^l_{t;\tau_k}(s,a) \!-\! W^{l-1}_{t;\tau_k}(s,a) \right)^2 \!+\! 2(W^{\min(T^A(s,a,\tau_k, t\!-\!1))}_{t;\tau_k}(s,a))^2  } \right)\\
    &\leq 2\exp\left( -\frac{\hat{\epsilon}^2\tau_k^{2\omega}}{2(|T^A(s,a,\tau_k,t-1)|+1)V_{\max}^2} \right) \overset{\text{(i)}}{\leq} 2\exp\left( -\frac{\tilde{\epsilon}^2\tau_k^{2\omega}}{2(t-\tau_k)V_{\max}^2} \right)\\
    &\leq 2\exp\left( -\frac{\tilde{\epsilon}^2\tau_k^{2\omega}}{2(\tau_{k+2}-\tau_k)V_{\max}^2} \right) 
    \overset{\text{(ii)}}{\leq} 2\exp\left( -\frac{\kappa^2\tilde{\epsilon}^2\tau_k^{\omega}}{8cL(cL+\kappa)V_{\max}^2} \right)\\
    &= 2\exp\left( -\frac{\kappa^2\tilde{\epsilon}^2\tau_k^{\omega}}{8cL(cL+\kappa)V_{\max}^2} \right),
\end{align*}
where (i) follows from Proposition \ref{prop:sa2L} and (ii) holds because
\begin{equation*}
    \tau_{k+2} - \tau_k = \frac{2cL}{\kappa}\tau_{k+1}^\omega + \frac{2cL}{\kappa}\tau_k^\omega = \frac{2cL}{\kappa}\left( \tau_k + \frac{2cL}{\kappa}\tau_k^\omega \right)^\omega + \frac{2cL}{\kappa}\tau_k^\omega \leq \frac{4cL(cL+\kappa)}{\kappa^2}\tau_k^\omega.
\end{equation*}

\textbf{Step 5: Taking union over all blocks }

% Now we put all the results obtained in previous steps together to get the conclusion of~\Cref{lem:conditionalBoundAsy}.
Applying the union bound in Lemma \ref{lem:unionBound}, we obtain
\begin{align*}
    &\mP\left[ \forall k\in [0,m], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^A_t  - Q^* }\leq D_{k+1}  | G,H\right]\\
    &\quad\geq \mP\left[ \forall(s,a), \forall k\in [0,m], \forall t\in[\tau_{k+1},\tau_{k+2}), \lvert W_{t;\tau_k}(s,a)  \rvert \leq \frac{\Delta}{2+\Delta}\beta D_k|G,H \right]\\
    &\quad\geq 1 - \sum_{k=0}^m |\mcs||\mca|(\tau_{k+2}-\tau_{k+1}) \cdot \mP\left[ \lvert W_{t;\tau_k}(s,a)  \rvert > \frac{\Delta}{2+\Delta}\beta D_k \Big\rvert t\in[\tau_{k+1},\tau_{k+2}),G,H  \right]\\
    &\quad\geq 1 - \sum_{k=0}^m |\mcs||\mca| \frac{2cL}{\kappa}\tau_{k+1}^\omega \cdot 2\exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 D_k^2\tau_k^{\omega}}{8cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\geq 1 - \sum_{k=0}^m |\mcs||\mca| \frac{2cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\tau_{k}^\omega \cdot 2\exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 D_k^2\tau_k^{\omega}}{8cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\overset{\text{(i)}}{\geq} 1 - \sum_{k=0}^m |\mcs||\mca| \frac{2cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\tau_{k}^\omega \cdot 2\exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 \epsilon^2\tau_k^{\omega}}{8cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\overset{\text{(ii)}}{\geq} 1 - \frac{4cL}{\kappa}\left(1+\frac{2cL}{\kappa}\right)\sum_{k=0}^m |\mcs||\mca| \cdot \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 \epsilon^2\tau_k^{\omega}}{16cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad\geq 1 - \frac{4cL(m+1)}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 \epsilon^2\tau_1^{\omega}}{16cL(cL+\kappa)V_{\max}^2} \right),
\end{align*}
where (i) follows because $D_k\geq D_m\geq \epsilon$, and (ii) follows from Lemma \ref{lem:tauHelp} by substituting $a=\frac{16cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\beta^2\epsilon^2 }, b=1$ and observing that
\begin{align*}
    \tau_k^{\omega}&\geq\hat{\tau}_1^{\omega}\geq \frac{32cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\beta^2\epsilon^2 }\ln\left(\frac{64cL(cL+\kappa)V_{\max}^2}{\kappa^2\left(\frac{\Delta}{2+\Delta}\right)^2\beta^2\epsilon^2 }\right)
    = 2ab\ln ab.
\end{align*}

\subsection{Part III: Bound $\norm{Q^A_t-Q^*}$}
In order to obtain the unconditional high-probability bound on $\norm{Q^A_t-Q^*}$, we first characterize a lower bound on the probability of Event $H$. Note that the probability of Event $G$ is lower bounded in~\Cref{lem:GqAsy}. 
\begin{lemma}\label{lem:halfQAAsy}
Let the sequence $\tau_k$ be the same as given in Lemma \ref{lem:coupleAsy}, i.e. $\tau_{k+1} = \tau_k + \frac{2cL}{\kappa}\tau_k^\omega$ for $k\geq 1$. Define $I^A_k$ as the number of iterations updating $Q^A$ at epoch $k$. Then we have
\begin{equation*}
    \mP\left[\forall k\in [1,m], I^A_k\geq cL\tau_{k}^\omega \right] \geq 1- m \exp\left( -\frac{(1-\kappa)^2cL\tau_1^\omega}{\kappa} \right).
\end{equation*}
\end{lemma}
\begin{proof}
We use the same idea as the proof of Lemma \ref{lem:halfQA}. Since we only focus on the blocks with $k\geq 1$, $I^A_k\sim Binomial\left( \frac{2cL}{\kappa}\tau_k^\omega, 0.5 \right)$ in such a case. Thus the tail bound of a binomial random variable gives
\begin{equation*}
    \mP \left[I^A_k\leq \frac{\kappa}{2}\cdot \frac{2cL}{\kappa}\tau_k^\omega\right] \leq \exp\left( -\frac{(1-\kappa)^2 cL\tau_k^\omega}{\kappa} \right).
\end{equation*}
Then by the union bound, we have
\begin{align*}
    \mP \left[\forall k\in[1,m], I^A_k\geq cL\tau_k^\omega\right]
    &=\mP \left[\forall k\in[1,m], I^A_k\geq \frac{\kappa}{2}\cdot \frac{2cL}{\kappa}\tau_k^\omega\right]\\
    &\geq 1 - \sum_{k=1}^m\exp\left( -\frac{(1-\kappa)^2 cL\tau_k^\omega}{\kappa} \right)\\
    &\geq 1- m \exp\left( -\frac{(1-\kappa)^2 cL\tau_1^\omega}{\kappa} \right).
\end{align*}
\end{proof}

Following from Lemma \ref{lem:totalIter}, it suffices to determine the starting time at epoch $m^*=\left\lceil \frac{4}{1-\gamma}\ln \frac{2\gamma V_{\max}}{\epsilon(1-\gamma)}\right\rceil$. This can be done by using Lemma \ref{lem:iteration} if we have $\hat{\tau}_1$.

Now we are ready to prove the main result of~\Cref{thm:asyncDQ}. By the definition of $m^*$, we know $D_{m^*-1}\geq\epsilon, G_{m^*-1}\geq \sigma\epsilon$. Then we obtain
\begin{align*}
    &\mP(\norm{Q^A_{\tau_{m^*}} - Q^* } \leq \epsilon)\\
    & \geq\mP\left[\forall k\in [0,m^* -1], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^A_t  - Q^* }\leq D_{k+1} \right]\\
    & = \mP\left[ \forall k\in [0,m^* -1], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^A_t  - Q^* }\leq D_{k+1} |G,H \right]\cdot\mP(G\cap H)\\
    & \geq \mP\left[ \forall k\in [0,m^* -1], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^A_t  - Q^* }\leq D_{k+1} |G,H \right]\\
    &\quad \cdot (\mP(G)+\mP(H)-1)\\
    &\overset{\text{(i)}}{\geq}\mP\left[ \forall k\in [0,m^* -1], \forall t\in[\tau_{k+1},\tau_{k+2}), \norm{Q^A_t  - Q^* }\leq D_{k+1} |G,H \right]\\
    &\quad\cdot \left(\mP\left[ \forall q\in [0, m^* -1], \forall t\in[\hat{\tau}_{q+1},\hat{\tau}_{q+2}), \norm{Q^B_t  - Q^A_t }\leq G_{q+1} \right] + \mP(H) - 1\right)\\
    &\overset{\text{(ii)}}{\geq}\left[ 1 - \frac{4cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 \epsilon^2\tau_1^{\omega}}{16cL(cL+\kappa)V_{\max}^2} \right) \right]\\
    &\quad\cdot\left[ 1- \frac{4cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64cL(cL+\kappa)V_{\max}^2} \right)\right.\\
    &\quad\quad \left.- m^*\! \exp\!\left( -\frac{(1 -\kappa)^2 cL\hat{\tau}_1^{\omega}}{\kappa} \right) \right]\\
    &\geq 1- \frac{4cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\beta^2 \epsilon^2\tau_1^{\omega}}{16cL(cL+\kappa)V_{\max}^2} \right)\\
    &\quad - \!\frac{4cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64cL(cL+\kappa)V_{\max}^2} \right)\! -\! m^* \exp\left( -\frac{(1\!-\!\kappa)^2 cL\hat{\tau}_1^{\omega}}{\kappa} \right)\\
    &\overset{\text{(iii)}}{\geq} 1- \frac{12cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2(1-\kappa)^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64 cL(cL+\kappa)V_{\max}^2} \right),
\end{align*}
where (i) follows from~\Cref{lem:coupleAsy}, (ii) follows from Propositions \ref{lem:GqAsy} and \ref{lem:conditionalBoundAsy} and (iii) holds due to the fact that
\begin{align*}
    \frac{4cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| = \max&\left\{ \frac{4cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca|, m^* \right\},\\
    \frac{\kappa^2(1\!-\!\kappa)^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64cL(cL+\kappa)V_{\max}^2}\!\leq\! \min&\left\{ \frac{\kappa^2\!\left( \frac{\Delta}{2+\Delta} \right)^2\!\beta^2 \epsilon^2\hat{\tau}_1^{\omega}}{16cL(cL+\kappa)V_{\max}^2}, \frac{(1\!-\!\kappa)^2\hat{\tau}_1^{\omega}}{\kappa}, \frac{\kappa^2\!\left( \frac{\Delta}{2+\Delta} \right)^2\!\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64cL(cL+\kappa)V_{\max}^2}\right\}.
\end{align*}
% where the second inequality holds since $\omega\in[1/2,1), \kappa\in[1/2,1)$.

By setting 
\begin{equation*}
    1- \frac{12cLm^*}{\kappa}\left(1+\frac{2cL}{\kappa}\right)|\mcs||\mca| \exp\left( -\frac{\kappa^2(1-\kappa)^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2\hat{\tau}_1^{\omega}}{64 cL(cL+\kappa)V_{\max}^2} \right) \geq 1-\delta,
\end{equation*}
we obtain
\begin{equation*}
    \hat{\tau}_1 \geq \left( \frac{64 cL(cL+\kappa)V_{\max}^2}{\kappa^2(1-\kappa)^2\left( \frac{\Delta}{2+\Delta} \right)^2\xi^2 \sigma^2\epsilon^2}\ln \frac{12m^*|\mcs||\mca|cL(2cL+\kappa)}{\kappa^2\delta} \right)^{\frac{1}{\omega}}.
\end{equation*}

Combining with the requirement of $\hat{\tau}_1$ in Propositions \ref{lem:GqAsy} and \ref{lem:conditionalBoundAsy}, we can choose 
\begin{equation*}
    \hat{\tau}_1 = \Theta\left( \left(\frac{ L^4V_{\max}^2}{(1-\gamma)^4\epsilon^2}\ln \frac{ m^*|\mcs||\mca|L^4V_{\max}^2}{(1-\gamma)^4\epsilon^2\delta} \right)^{\frac{1}{\omega}} \right).
\end{equation*}

Finally, applying $m^*=\left\lceil\frac{4}{1-\gamma}\ln \frac{2\gamma V_{\max}}{\epsilon(1-\gamma)}\right\rceil$ and Lemma \ref{lem:iteration}, we conclude that it suffices to let
\begin{align*}
    T&=\Omega\left( \left(\frac{ L^4V_{\max}^2}{(1-\gamma)^4\epsilon^2}\ln \frac{m^*|\mcs||\mca|L^4V_{\max}^2}{(1-\gamma)^4\epsilon^2\delta} \right)^{\frac{1}{\omega}} + \left(\frac{2cL}{\kappa}\frac{1}{1-\gamma} \ln\frac{\gamma V_{\max}}{(1-\gamma)\epsilon} \right)^{\frac{1}{1-\omega}} \right)\\
    &=\Omega\left( \left(\frac{ L^4V_{\max}^2}{(1-\gamma)^4\epsilon^2}\ln \frac{|\mcs||\mca|L^4V_{\max}^2 \ln \frac{2\gamma V_{\max}}{\epsilon(1-\gamma)}}{(1-\gamma)^5\epsilon^2\delta} \right)^{\frac{1}{\omega}} + \left(\frac{2cL}{\kappa}\frac{1}{1-\gamma} \ln\frac{\gamma V_{\max}}{(1-\gamma)\epsilon} \right)^{\frac{1}{1-\omega}} \right)\\
    &=\Omega\left( \left(\frac{ L^4V_{\max}^2}{(1-\gamma)^4\epsilon^2}\ln \frac{|\mcs||\mca|L^4V_{\max}^2 }{(1-\gamma)^5\epsilon^2\delta} \right)^{\frac{1}{\omega}} + \left(\frac{L^2}{1-\gamma} \ln\frac{\gamma V_{\max}}{(1-\gamma)\epsilon} \right)^{\frac{1}{1-\omega}} \right).
\end{align*}
to attain an $\epsilon$-accurate Q-estimator.





